Streaming4D: Accelerate 4D World Models via Block-wise Video Generation and Incremental Reconstruction

Current 4D generation paradigms are often bottlenecked by a sequential decoupling design: video is generated first, followed by 3D reconstruction, leading to high interaction latency. This limits applications in interactive real-time scenarios. To this end, we propose \textbf{Streaming4D}, a tightly coupled synchronous pipeline that integrates block-wise autoregressive video generation with incremental 3D reconstruction. Unlike traditional frame-by-frame emission and delayed geometry recovery, Streaming4D generates temporal video blocks and immediately triggers reconstruction for each completed block, enabling parallel execution between synthesis and geometric updates. This approach allows the world representation to evolve online with the video stream, reducing feedback latency while preserving geometric fidelity. We instantiate \textbf{Streaming4D} using a Self-Forcing-style autoregressive generator and an incremental reconstruction backend. Experiments show consistent runtime improvements across resolutions on a single RTX 4090 (1.24$\times$ speedup), while maintaining high-quality 4D geometry and multi-view consistency.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/5_analysis.tex <==
\section{Analysis}

\textbf{Quantitative and Qualitative Studies.} 
% Table~\ref{tab:comparison} shows our method outperforms others across all metrics (mPSNR, mSSIM, mLPIPS), indicating strong feature preservation, multi-scale representation, and temporal consistency. SeVA's poor results highlight its limitations, while Megasam's second place suggests its rendering lacks temporal stability. In Figure~\ref{fig:qualitive}, our method demonstrates superior geometric accuracy (e.g., intact structures in indoor scenes) and temporal coherence (in urban sequences), with clear improvements in structural completeness, motion smoothness, and multi-view consistency. Competitors exhibit artifacts like structural gaps (Shape-of-Motion), blur (Cut3rR), or flickering (Megasam), confirming our advantage in joint geometry and motion modeling.
Based on the experimental results presented in the previous section, our analysis reveals the key strengths of the proposed approach. The superior performance of our method is not merely reflected in quantitative gains or visual quality, but fundamentally stems from its ability to jointly model geometry and dynamics while maintaining multi-view and temporal consistency. The analysis highlights how architectural choices—such as the integration of pose-aware warping and dynamic feature refinement—directly address common failure modes in existing methods, such as structural fragmentation, motion blur, and flickering. By examining both numerical trends and visual artifacts across baselines, we identify that competing approaches often sacrifice one aspect of reconstruction quality (e.g., geometry) for another (e.g., smoothness), whereas our design enables synergistic improvements. 

% \textbf{Quantitative Study.} Our performance comparison \ref{tab:comparison} shows fundamental advantages in 4D reconstruction. Our method leads across all metrics (mPSNR, mSSIM, mLPIPS), demonstrating successful balance between feature preservation, multi-scale representation, and temporal consistency. SeVA's poor performance reveals framework limitations, while Megasam's second place shows its neural rendering still lacks temporal coherence. Unlike approaches that trade off between metrics, our method maintains consistent superiority, proving our architectural innovations create synergistic improvements across all dimensions.

% The performance comparison table reveals fundamental differences in how various 4D reconstruction approaches handle the complex task of spatiotemporal modeling. The superior performance of our method across all metrics suggests that its architectural design successfully addresses several key challenges inherent to 4D reconstruction. This consistent performance across metrics suggests our method has achieved an optimal balance between several competing demands: the network's feature preservation mechanisms (reflected in mPSNR) work synergistically with its multi-scale representation strategy (captured by mSSIM) to overcome the temporal inconsistency problems that typically degrade perceptual quality (measured by mLPIPS). The particularly poor performance of SeVA across all metrics suggests fundamental limitations in its basic framework for handling dynamic elements, while Megasam's second-place position indicates that its neural rendering approach, while competent, still misses important aspects of temporal coherence that our method captures. The intermetric consistency confirms that our architectural innovations do not simply optimize for one aspect of reconstruction at the expense of others, but rather create a virtuous cycle. This holistic advancement explains why our method maintains its performance lead across all evaluation dimensions, setting it apart from approaches that may excel in one metric while compromising others.

% \noindent
% \textbf{Qualitative Study.} Figure \ref{fig:qualitive} compares four 4D reconstruction methods (Ours, Shape-of-Motion, Cut3rR, Megasam) across static and dynamic scenes. The upper quadrant evaluates geometric accuracy (indoor scene with furniture), while the lower quadrant tests temporal consistency (urban street sequences). Input-output pairs with green annotations highlight key differences in: (1) structural completeness (intact walls/furniture in our results), (2) dynamic handling (coherent motion), and (3) multi-view consistency (green camera frustums). Our method excels in spatial detail and temporal coherence, while competitors show structural degradation (Shape-of-Motion), blur (Cut3rR), or flickering (Megasam). These results demonstrate our approach's superiority in joint geometry and motion modeling.

% Figure \ref{fig:qualitive} provides a comprehensive visual assessment of four leading 4D reconstruction approaches (Ours, Shape-of-Motion, Cut3rR, and Megasam) through systematic comparison across both spatial and temporal dimensions.    The upper ``Static Scene" quadrant evaluates geometric reconstruction quality using an indoor living space (featuring a red sofa and surrounding furniture), while the lower ``Dynamic Scene" quadrant examines temporal consistency through urban street sequences. Each method's output is juxtaposed with its corresponding input frame (left panels), with green annotations strategically placed to emphasize critical performance differences in: (1) structural completeness (notice the intact walls and furniture contours in our results), (2) dynamic element handling (observe the coherent motion trajectories in street scenes), and (3) multi-view consistency (evident from the green camera frustums indicating evaluation viewpoints). The visualization particularly highlights our method's dual advantage in preserving fine spatial details while maintaining temporal coherence, with competing approaches showing varying degrees of structural degradation (Shape-of-Motion), blur artifacts (Cut3rR), or temporal flickering (Megasam). These qualitative findings collectively demonstrate how our architectural innovations address the core challenges of simultaneous geometry reconstruction and motion modeling in understanding 4D scenes.

% Megasam demonstrates good texture fidelity in static scenes, but it has obvious timing jitter problems during dynamic reconstruction. The geometric structure of Shape-of-Motion is relatively complete, but the restoration of detailed textures is weak, resulting in a blurred surface. Cut3r performs stably in simple scenes, but local distortion and motion artifacts may occur in complex dynamic scenes. In contrast, our method demonstrates superior comprehensive performance in terms of geometric accuracy, texture detail and temporal consistency.

\noindent
\textbf{Ablation Study.} The experimental results of ablation study are presented in Table x and Figure x. The dynamic approaches (Dynamic Module + 4D Generator) achieve the best performance across all metrics (mPSNR: 19.78 dB, mSSIM: 0.6686, mLPIPS: 0.1220), demonstrating the synergistic effect of integrating dynamic generation with 4D reconstruction. Removing the 4D Generator (Only Dynamic Module) leads to significant degradation. For dynamic sequences, the gain of the 4D Generator of 1.41 dB mPSNR and the reduction of $33.7\%$ mLPIPS 
% (0.1841 0.1220) 
(0.1841 $\to$ 0.1220)
demonstrate its ability to resolve temporal inconsistencies that pure diffusion-based generation cannot eliminate alone. The module achieves this through: (1) geometry-aware refinement that corrects shape drift accumulated across frames using 3D consistency constraints, and (2) temporal feedback loops that iteratively align surface details with reconstructed 4D geometry. 
% This explains why dynamic models benefit more from 4D integration than static ones (+1.41 dB vs +0.79 dB mPSNR) - their inherent motion coherence provides stronger geometric priors for the 4D Generator to exploit. 
This suggests that dynamic inputs provide richer spatiotemporal cues (coherent motion patterns) that the 4D Generator utilizes more effectively than static inputs (only viewpoint variation). For static models, the smaller improvements (0.79 dB mPSNR, 0.0771 mSSIM) reveal their architectural limitation: lacking motion modeling, they depend entirely on the 4D Generator to compensate for viewpoint disparities, acting primarily as a geometric corrector.

% dynamic inputs, which contain coherent motion patterns, provide richer spatiotemporal cues that the 4D Generator can leverage more effectively than static inputs, where only viewpoint variation is available.
% For static models, the more modest 0.79 dB mPSNR and 0.0771 mSSIM improvement reveal their architectural limitation: Without motion modeling, they rely entirely on the 4D Generator to compensate for large viewpoint disparities. These gains reveal the role of the module as a geometric corrector, enforcing multi-view consistency when the static architecture alone performs poorly.

% In addition to the objective comparison in terms of quantity, the ablation research has intuitively demonstrated the crucial role of the 4D generator in achieving spatiotemporal consistency in both dynamic and static scenes. 

Beyond quantitative comparisons, the ablation study visually demonstrates the critical role of the 4D Generator in achieving spatiotemporal consistency. Figure x demonstrates the 4D Generator's crucial role in spatiotemporal consistency. The dynamic baseline (upper left) produces discontinuous seagull motion, while the static version (upper right) fails to maintain viewpoint consistency. Our 4D Generator (bottom row) significantly improves both: enabling smooth bird flight paths (bottom left) and coherent multi-view geometry (bottom right). In particular, it simultaneously ensures (1) temporal smoothness (seagull sequence \ding{172} $\rightarrow$ \ding{173} $\rightarrow$ \ding{174}) and (2) spatial integrity (consistent furniture across views \ding{172} $\rightarrow$ \ding{175}). This confirms the 4D Generator fundamentally enhances spatiotemporal reasoning, bridging discrete 3D reconstruction and continuous 4D modeling.

% Beyond quantitative comparisons, the ablation study visually demonstrates the critical role of the 4D Generator in achieving spatiotemporal consistency.
% As shown in Figure \ref{fig:ablation}, the dynamic baseline module (upper left) produces discontinuous motion trajectories for seagulls, while its static counterpart (upper right) fails to maintain viewpoint consistency in the indoor scene.   The introduction of our 4D Generator (bottom row) yields significant improvements: the enhanced dynamic module (bottom left) now generates physically plausible bird flight paths with proper temporal interpolation, and the upgraded static module (bottom right) achieves multi-view coherence in room geometry reconstruction.   Particularly noteworthy is the 4D Generator's dual capability to simultaneously handle: (1) temporal smoothness in dynamic elements (evident in the seagull sequence \ding{172} $\rightarrow$ \ding{173} $\rightarrow$ \ding{174}) and (2) spatial integrity across viewpoints (demonstrated by the consistent furniture arrangement in views \ding{172} $\rightarrow$ \ding{175}).   These visual comparisons confirm that the 4D Generator is not merely an additive component but fundamentally transforms both modules' capacity for spatiotemporal reasoning, bridging the gap between discrete 3D reconstruction and continuous 4D scene modeling.

% The multi-view and temporal consistency of our generated sequences forms the foundation for producing high-quality 4D scene reconstructions, as demonstrated through extensive comparative analysis. By establishing a bidirectional coupling between the camera-controlled video generation pipelines (Section 3.2) and 4D reconstruction pipelines (Section 3.3), our approach successfully maintains spatiotemporal consistency across both modules. This is particularly evident in challenging scenarios involving complex occlusions and non-rigid deformations, where our method demonstrates significantly improved robustness compared to single-modality approaches. The quantitative and qualitative evaluations confirm that our temporal-aware geometry optimization strategy effectively addresses the shape drift and flickering issues that commonly plague 4D generation methods, while the unified camera control mechanism enables precise viewpoint manipulation without compromising dynamic consistency.
Together, these results validate the effectiveness of our bidirectional design in maintaining spatiotemporal coherence, particularly under complex occlusions and non-rigid motions.

==> table1.tex <==
\begin{table*}[t]
\centering
\caption{A two-column table.}
\label{tab:table8}
\small % 或 \footnotesize，根据实际宽度调整
\setlength{\tabcolsep}{3.5pt} % 默认是 6pt，减小以节省空间
\renewcommand{\arraystretch}{1.1} % 稍微增加行高，提升可读性
\begin{tabular}{c|*{4}{c}|*{4}{c}|*{4}{c}|*{4}{c}|*{4}{c}}
\hline
 & \multicolumn{4}{c|}{Glass} 
 & \multicolumn{4}{c|}{Object A} 
 & \multicolumn{4}{c|}{Object B} 
 & \multicolumn{4}{c|}{Object C}  
 & \multicolumn{4}{c}{Average} \\
\cline{2-5} \cline{6-9} \cline{10-13} \cline{14-17} \cline{18-21}
 & F-EPE & A-MSE & I-MSE & M-IoU 
 & F-EPE & A-MSE & I-MSE & M-IoU 
 & F-EPE & A-MSE & I-MSE & M-IoU 
 & F-EPE & A-MSE & I-MSE & M-IoU 
 & F-EPE & A-MSE & I-MSE & M-IoU \\
\hline
Method A & 3.6 / 30.3 & 1.33 & 0.48 & 0.12 & 6.4 / 53.2 & 1.54 & 0.68 & 0.12 & 10.3 / 39.2 & 1.94 & 1.57 & 0.24 & 6.8 / 56.8 & 2.50 & 0.85 & 0.11 & 6.8 / 44.9 & 1.83 & 0.90 & 0.15 \\
Method B & 2.1 / 15.8 & 0.22 & 0.14 & 0.97 & 3.1 / 23.5 & 0.31 & 0.23 & 0.97 & 2.0 / 6.7   & 0.17 & 0.28 & 0.99 & 4.5 / 34.4 & 0.38 & 0.33 & 0.92 & 2.9 / 20.1 & 0.27 & 0.24 & 0.96 \\
\hline
Method C & 1.9 / 14.7 & 0.21 & 0.14 & 0.97 & 2.9 / 21.8 & 0.30 & 0.22 & 0.97 & 1.9 / 6.6   & 0.15 & 0.29 & 0.99 & 4.1 / 31.5 & 0.37 & 0.32 & 0.92 & 2.7 / 18.6 & 0.26 & 0.24 & 0.96 \\
\hline
\end{tabular}
\end{table*}
